Conversable Quantum Fire in the Standard Model

Quantum fire consists of quantum states that can be efficiently functionally cloned but cannot be transmitted using one-way classical communication. Whereas all previous quantum-fire constructions with proven untelegraphability are relative to an oracle, ours, based on one-shot signatures, is in the standard model. Our construction achieves two further notions that we introduce: (a) keyless untelegraphability, a strengthening of untelegraphability; and (b) conversability, meaning that a flame, though not telegraphable via one-way classical communication, can be transmitted via classical interaction. Hence one-way and two-way classical communication differ qualitatively in their power to transmit this quantum fire. We use these two novel properties of quantum fire, along with its clonability, to give one of the first cryptographic applications of quantum fire. Keyless untelegraphability forces the distribution of serial numbers of valid flames to have high min-entropy, while conversability and clonability allow the corresponding flame to be cloned and transferred using only classical communication. We present two variants of our conversable quantum-fire construction. The first, based on one-shot signatures (instantiable from subexponential iO, subexponentially secure one-way functions, and LWE), supports polynomially many flames, and super-logarithmic min-entropy of the serial-number distribution. The second, under the stronger assumption of exponentially unforgeable one-shot signatures (instantiable relative to a classical oracle), supports exponentially many flames, and linear min-entropy.

==> figs/images/construction/clone/clone-figure.tex <==
% Reusable Clone drawing. Its caller supplies TikZ, graphicx, the required
% libraries, and the Yoav illustration primitives.
\begingroup
\newcommand{\yoavfigclone}{\mathpzc{Clone}}
\newcommand{\yoavfigclonespark}{\mathpzc{Spark}}
\newcommand{\yoavfigclonesign}{\mathsf{OSS.Sign}}

\definecolor{constructionblue}{RGB}{45,55,210}
\definecolor{constructionred}{RGB}{206,44,45}
\definecolor{constructionyellow}{RGB}{240,185,0}

% A verification-key square and its matching one-shot quantum signing token.
\newcommand{\yoavfigclonekeytokenpair}[1]{%
  \ensuremath{\Bigl(
    \coloredsquare[0.40cm]{#1},\;
    \left|\,\signingstamp{#1}\,\right\rangle
  \Bigr)}%
}

\scalebox{1.20}{%
\begin{tikzpicture}[
  stage arrow/.style={-{Stealth[length=3.1mm,width=2.0mm]},
                      draw=black!72, line width=0.95pt,
                      dash pattern=on 4pt off 3pt, line cap=round},
  tree edge/.style={draw=black!68, line width=0.85pt,
                    line cap=round},
  stage object/.style={inner sep=1pt, outer sep=0pt},
  operation label/.style={anchor=west, inner sep=1pt, outer sep=0pt,
                          font=\yoavlabeltext},
  state outline/.style={draw=black, line width=1.35pt,
                        line cap=round, line join=round}
]
  % Algorithm heading. Everything after the colon is indented.
  \node[anchor=west, inner sep=0pt] at (0,19.70)
    {$\yoavfigclone\!\left(
       \coloredsquare[0.34cm]{constructionblue},\;
       \livesigningtokenindex{constructionblue}{constructionblue}
     \right)\mathpunct{:}$};

  % Stage 1: the supplied flame.
  \node[stage object] (input) at (4.25,17.75)
    {\yoavfigclonekeytokenpair{constructionblue}};

  % Generate the two fresh red/yellow OSS key-token pairs.
  \draw[stage arrow] (input.south) -- (4.25,15.06);
  \node[operation label] at (4.58,16.18)
    {$\yoavfigclonespark(1^\lambda)^{\otimes 2}$};

  % Stage 2: retain the original blue flame and display both fresh children.
  \node[stage object] (retained) at (4.25,14.25)
    {\yoavfigclonekeytokenpair{constructionblue}};
  \node[stage object] (fresh red) at (2.38,12.05)
    {\yoavfigclonekeytokenpair{constructionred}};
  \node[stage object] (fresh yellow) at (6.12,12.05)
    {\yoavfigclonekeytokenpair{constructionyellow}};

  % The second stage is an undirected three-node tree.
  \draw[tree edge] (retained.south) -- (fresh red.north);
  \draw[tree edge] (retained.south) -- (fresh yellow.north);

  % Consume the blue token to sign the ordered pair of fresh public keys.
  \draw[stage arrow] (4.25,11.24) -- (4.25,9.70);
  \node[operation label] at (4.58,10.22) {$
    \yoavfigclonesign\!\bigl(
      \left|\,\signingstamp{constructionblue}\,\right\rangle,\;
      \coloredsquare[0.31cm]{constructionred}\;
      \coloredsquare[0.31cm]{constructionyellow}
    \bigr)
  $};

  % Stage 3: the signed binary-tree link shared by the two output flames.
  \node[stage object] (root key) at (4.25,8.25)
    {\coloredsquare[0.46cm]{constructionblue}};
  \node[stage object] (signed link) at (4.25,6.05)
    {\scalebox{1.12}{\signedkeypair
      {constructionblue}{constructionred}{constructionyellow}}};
  \node[stage object] (left output) at (1.93,3.10)
    {\yoavfigclonekeytokenpair{constructionred}};
  \node[stage object] (right output) at (6.57,3.10)
    {\yoavfigclonekeytokenpair{constructionyellow}};

  \draw[tree edge] (root key.south) -- (signed link.north);
  \draw[tree edge] (signed link.south west) -- (left output.north east);
  \draw[tree edge] (signed link.south east) -- (right output.north west);

  % Oppositely tilted ellipses make the two descendant states explicit.
  % Each excludes the shared root and contains the certificate and one child.
  \begin{scope}[on background layer]
    \begin{scope}[shift={(3.12,4.25)}, rotate=66]
      \draw[state outline] (0,0)
        ellipse [x radius=3.75cm, y radius=2.35cm];
    \end{scope}
    \begin{scope}[shift={(5.38,4.25)}, rotate=-58]
      \draw[state outline] (0,0)
        ellipse [x radius=3.75cm, y radius=2.35cm];
    \end{scope}
  \end{scope}

  % The original serial number is the fire index of both cloned states.
  \node[inner sep=0pt, outer sep=0pt] at (2.08,0.21)
    {\scalebox{0.46}{\fireglyph{constructionblue}}};
  \node[inner sep=0pt, outer sep=0pt] at (6.72,0.48)
    {\scalebox{0.46}{\fireglyph{constructionblue}}};
\end{tikzpicture}%
}%
\endgroup


==> figs/images/construction/converse/converse-figure.tex <==
% Reusable Converse drawing. Its caller supplies TikZ, graphicx, the required
% libraries, and the Yoav illustration primitives.
\begingroup
\newcommand{\yoavconverseverify}{\mathpzc{Verify}}
\newcommand{\yoavconverseossgen}{\mathsf{OSS.Gen}}
\newcommand{\yoavconverseosskeygen}{\mathsf{OSS.KeyGen}}
\newcommand{\yoavconverseosssign}{\mathsf{OSS.Sign}}

\definecolor{constructionblue}{RGB}{45,55,210}
\definecolor{constructionred}{RGB}{206,44,45}
\definecolor{constructiongreen}{RGB}{42,177,72}

% All readable text in this illustration uses a 16-point baseline.
\renewcommand{\yoavlabeltext}{\fontsize{16pt}{19.2pt}\selectfont}

% A verification-key square and its matching one-shot quantum signing token.
\newcommand{\yoavconversekeytokenpair}[1]{%
  \ensuremath{\Bigl(
    \coloredsquare[0.40cm]{#1},\;
    \left|\,\signingstamp{#1}\,\right\rangle
  \Bigr)}%
}

% The initial state carries the blue fire as its serial-number index.
\newcommand{\yoavconverselivekeytokenpair}[1]{%
  \ensuremath{\Bigl(
    \coloredsquare[0.40cm]{#1},\;
    \livesigningtokenindex{#1}{#1}
  \Bigr)}%
}

% The authenticated prefix transmitted from Alice to Bob.
\newcommand{\yoavconversetransmittedpath}[1][0.62]{%
  \ensuremath{\Bigl(
    \coloredsquare[0.27cm]{constructionblue},\;
    \signedkeypair[#1]
      {constructionblue}{constructiongreen}{constructionred}
  \Bigr)}%
}

% Bob completes the received prefix with his red terminal key. This is the
% three-entry path passed as Verify's first argument.
\newcommand{\yoavconverseverificationpath}[1][0.48]{%
  \ensuremath{\Bigl(
    \coloredsquare[0.27cm]{constructionblue},\;
    \signedkeypair[#1]
      {constructionblue}{constructiongreen}{constructionred},\;
    \coloredsquare[0.27cm]{constructionred}
  \Bigr)}%
}

\scalebox{1.20}{%
\begin{tikzpicture}[
  font=\yoavlabeltext,
  object/.style={inner sep=1pt, outer sep=0pt},
  formula/.style={inner sep=0pt, outer sep=0pt, font=\yoavlabeltext},
  tree edge/.style={draw=black!68, line width=0.90pt,
                    line cap=round, line join=round},
  state outline/.style={draw=black, line width=1.35pt,
                        line cap=round, line join=round},
  message arrow/.style={-{Stealth[length=3.2mm,width=2.2mm]},
                        draw=black!72, line width=1.05pt,
                        line cap=round}
]
  % Alice and Bob share one classical channel, displayed once before the
  % protocol begins. Time continues from top to bottom at the right.
  \node[font=\yoavlabeltext\sffamily] at (3.60,32.20) {Alice};
  \node[font=\yoavlabeltext\sffamily] at (17.40,32.20) {Bob};
  \node[object] at (10.50,32.20)
    {\ethernetcable[width=6.00cm, arrow=double, arrow span=0.58]};
  \node[anchor=north, inner sep=0pt, outer sep=0pt] at (22.15,32.40)
    {\timearrow[31.40cm]};

  % Alice first holds the blue live state.
  \node[object] at (1.85,28.35)
    {\yoavconverselivekeytokenpair{constructionblue}};

  % Bob then creates the red one-shot signing key and token.
  \node[formula, anchor=west] at (13.10,26.20) {$
    \yoavconversekeytokenpair{constructionred}
    \;\longleftarrow\;\yoavconverseosskeygen(1^\lambda)
  $};

  % Bob sends his red verification key to Alice.
  \draw[message arrow] (15.25,24.05) --
    node[midway, above=0.38cm, object]
      {\coloredsquare[0.31cm]{constructionred}}
    (5.75,24.05);

  % Alice creates the green pair.
  \node[formula, anchor=west] at (0.35,21.85) {$
    \yoavconversekeytokenpair{constructiongreen}
    \;\longleftarrow\;\yoavconverseossgen(1^\lambda)
  $};

  % On the following line Alice signs the ordered green/red children.
  \node[object] at (1.25,19.65)
    {\signedkeypair[1.02]
      {constructionblue}{constructiongreen}{constructionred}};
  \node[formula, anchor=west] at (2.28,19.65) {$
    \longleftarrow\;\yoavconverseosssign\!\left(
      \left|\,\signingstamp{constructionblue}\,\right\rangle,\;
      \coloredsquare[0.28cm]{constructiongreen}\;
      \coloredsquare[0.28cm]{constructionred}
    \right)
  $};

  % Alice sends the authenticated blue-rooted prefix to Bob.
  \draw[message arrow] (5.75,17.35) --
    node[midway, above=0.34cm, object]
      {\yoavconversetransmittedpath[0.72]}
    (15.25,17.35);

  % Bob verifies the received path against his red terminal key/token pair.
  \node[formula, anchor=west] at (14.05,15.25) {$
    \yoavconverseverify\!\left(
      \yoavconverseverificationpath[0.48],\;
      \left|\,\signingstamp{constructionred}\,\right\rangle
    \right)
  $};

  % The shared authenticated fork underlying the two final states.
  \node[object] (blue root) at (3.80,15.25)
    {\coloredsquare[0.46cm]{constructionblue}};
  \node[object] (signed link) at (3.80,12.05)
    {\signedkeypair[1.06]
      {constructionblue}{constructiongreen}{constructionred}};
  \node[object] (alice output) at (1.75,4.05)
    {\yoavconversekeytokenpair{constructiongreen}};
  \node[object] (bob output) at (17.40,4.05)
    {\yoavconversekeytokenpair{constructionred}};

  \draw[tree edge] (blue root.south) -- (signed link.north);
  \draw[tree edge] (signed link.south west) -- (alice output.north east);
  \draw[tree edge] (signed link.south east) -- (bob output.north west);

  % As in Clone, each contour excludes the shared root while containing the
  % certificate and one terminal child. The right-hand state spans Alice/Bob.
  \begin{scope}[on background layer]
    \begin{scope}[shift={(2.78,7.20)}, rotate=79]
      \draw[state outline] (0,0)
        ellipse [x radius=6.45cm, y radius=2.35cm];
    \end{scope}
    \begin{scope}[shift={(10.58,8.20)}, rotate=-29]
      \draw[state outline] (0,0)
        ellipse [x radius=9.85cm, y radius=2.75cm];
    \end{scope}
  \end{scope}

  % Both final states retain the original blue-fire serial number.
  \node[inner sep=0pt, outer sep=0pt] at (2.82,0.90)
    {\scalebox{0.68}{\fireglyph{constructionblue}}};
  \node[inner sep=0pt, outer sep=0pt] at (18.65,2.70)
    {\scalebox{0.68}{\fireglyph{constructionblue}}};
\end{tikzpicture}%
}%
\endgroup


==> figs/images/construction/spark/spark-figure.tex <==
% Reusable Spark drawing. Its caller supplies TikZ, graphicx, the required
% libraries, and the Yoav illustration primitives.
\begingroup
\newcommand{\yoavfigspark}{\mathpzc{Spark}}
\newcommand{\yoavfigsparkkeygen}{\mathsf{OSS.KeyGen}}
\definecolor{constructionblue}{RGB}{45,55,210}

\scalebox{1.20}{%
\begin{tikzpicture}
  \node[anchor=west, inner sep=0pt] at (0,1.00)
    {$\yoavfigspark(1^\lambda)\mathpunct{:}$};

  \node[anchor=west, inner sep=0pt] at (0.62,0) {$
    \Bigl(
      \coloredsquare[0.38cm]{constructionblue},\;
      \livesigningtokenindex{constructionblue}{constructionblue}
    \Bigr)
    \;\longleftarrow\;\yoavfigsparkkeygen(1^\lambda)
    $
  };
\end{tikzpicture}%
}%
\endgroup


==> figs/images/construction/verify/verify-figure.tex <==
% Reusable Verify drawing. Its caller supplies TikZ, graphicx, the required
% libraries, and the Yoav illustration primitives.
\begingroup
\newcommand{\yoavfigverify}{\mathpzc{Verify}}
\newcommand{\yoavfigverifysignature}{\mathsf{VerifySignature}}
\newcommand{\yoavfigverifytoken}{\mathsf{VerifyToken}}

\definecolor{constructionblue}{RGB}{45,55,210}
\definecolor{constructionred}{RGB}{206,44,45}
\definecolor{constructionyellow}{RGB}{240,185,0}
\definecolor{constructiongreen}{RGB}{42,177,72}
\definecolor{constructionpurple}{RGB}{132,62,166}

% All readable text in this illustration uses a 16-point baseline.
\renewcommand{\yoavlabeltext}{\fontsize{16pt}{19.2pt}\selectfont}

\newcommand{\yoavfigverifykeytokenpair}[1]{%
  \ensuremath{\Bigl(
    \coloredsquare[0.40cm]{#1},\;
    \left|\,\signingstamp{#1}\,\right\rangle
  \Bigr)}%
}

\scalebox{1.20}{%
\begin{tikzpicture}[
  font=\yoavlabeltext,
  path edge/.style={draw=black!68, line width=0.90pt,
                    line cap=round, line join=round},
  object/.style={inner sep=1pt, outer sep=0pt},
  check/.style={anchor=west, inner sep=0pt, outer sep=0pt},
  state outline/.style={draw=black, line width=1.35pt,
                        line cap=round, line join=round}
]
  % Verify the blue serial number against the blue-fire state.
  \node[anchor=west, inner sep=0pt] at (0,14.25) {$
    \yoavfigverify\!\left(
      \coloredsquare[0.40cm]{constructionblue},\;
      \firestate{constructionblue}
    \right)\mathpunct{:}
  $};

  % First authenticated link: blue signs the red/yellow pair.
  \node[object] (blue root) at (4.10,12.35)
    {\coloredsquare[0.46cm]{constructionblue}};
  \node[object] (first certificate) at (4.10,10.28)
    {\signedkeypair[1.12]
      {constructionblue}{constructionred}{constructionyellow}};
  \draw[path edge] (blue root.south) -- (first certificate.north);

  % Follow the yellow child to the second signed link.
  \node[object] (yellow key) at (5.33,8.48)
    {\coloredsquare[0.31cm]{constructionyellow}};
  \draw[path edge] (first certificate.south east) -- (yellow key.north west);

  % Second authenticated link: yellow signs the green/purple pair.
  \node[object] (second certificate) at (5.33,6.72)
    {\signedkeypair[1.12]
      {constructionyellow}{constructiongreen}{constructionpurple}};
  \draw[path edge] (yellow key.south) -- (second certificate.north);

  % Follow the green child to the terminal public key and quantum token.
  \node[object] (green terminal) at (3.58,4.32)
    {\yoavfigverifykeytokenpair{constructiongreen}};
  \draw[path edge] (second certificate.south west)
    -- (green terminal.north);

  % The ellipse contains the full authenticated path below, but not including,
  % the serial-number root. Its blue fire is shown as an index.
  \begin{scope}[on background layer]
    \begin{scope}[shift={(4.05,7.60)}, rotate=90]
      \draw[state outline] (0,0)
        ellipse [x radius=4.25cm, y radius=3.25cm];
    \end{scope}
  \end{scope}
  \node[inner sep=0pt, outer sep=0pt] at (5.25,3.16)
    {\scalebox{0.68}{\fireglyph{constructionblue}}};

  % Verify both certificates in path order. The trailing conjunction carries
  % into the terminal token check on the following indented line.
\node[check] at (0.62,1.4) {$
    \yoavfigverifysignature\!\left(
      \coloredsquare[0.25cm]{constructionblue},\;
      \vcenter{\hbox{\signedkeypair[0.56]
        {constructionblue}{constructionred}{constructionyellow}}}
      \hspace{0.42cm}
    \right)
    \;\wedge\;
    \yoavfigverifysignature\!\left(
      \coloredsquare[0.25cm]{constructionyellow},\;
      \vcenter{\hbox{\signedkeypair[0.56]
        {constructionyellow}{constructiongreen}{constructionpurple}}}
      \hspace{0.42cm}
    \right)
    \;\wedge
  $};

\node[check] at (1.06,0.0) {$
    \yoavfigverifytoken\!\Bigl(
      \coloredsquare[0.25cm]{constructiongreen},\;
      \left|\,\scalebox{0.56}{\signingstamp{constructiongreen}}\,\right\rangle
    \Bigr)
  $};
\end{tikzpicture}%
}%
\endgroup


==> figs/images/fire-security-game/fire-security-game-figure.tex <==
% Reusable keyless-untelegraphability game body.
\begingroup
\newcommand{\yoavgameverify}{\mathpzc{Verify}}
\definecolor{gameorange}{RGB}{242,122,24}

\begin{tikzpicture}
  % Level 1: adversary A initiates both classical messages.
  \node[draw=black!35, fill=white, rounded corners=1.5pt,
        inner sep=1.5pt, outer sep=0pt] (advA) at (0,6.70)
    {\includegraphics[height=1.50cm]{\yoavdatapath boyPirate}};
  \node[anchor=south, font=\yoavlabeltext] at (advA.north)
    {Adversary $\mathcal A$};

  % Level 2: adversary B receives the recipe, then prepares the fire state.
  \node[draw=black!35, fill=white, rounded corners=1.5pt,
        inner sep=1.5pt, outer sep=0pt] (advB) at (3.60,3.00)
    {\includegraphics[height=1.70cm]{\yoavdatapath girlPirate}};
  \node[anchor=north, yshift=-0.16cm, font=\yoavlabeltext] at (advB.south)
    {Adversary $\mathcal B$};

  % Level 3: the referee receives one message from each adversary.
  \node[draw=black!35, fill=white, rounded corners=1.5pt,
        inner sep=1.5pt, outer sep=0pt] (referee) at (-3.05,0.55)
    {\includegraphics[height=1.75cm]{\yoavdatapath referee}};
  \node[anchor=south, yshift=0.16cm, font=\yoavlabeltext] at (referee.north)
    {Referee};

  % A sends the orange serial number directly to the referee.
  \node[inner sep=0pt, outer sep=0pt] at (-1.43,3.40)
    {\ethernetcable[width=4.55cm, image height=0.40cm,
                    angle=-109, arrow=single,
                    arrow span=0.34]};
  \node[inner sep=0pt, outer sep=0pt] at (-2.20,3.95)
    {\coloredsquare[0.36cm][-109]{gameorange}};

  % At the same first level, A sends B a recipe for the coloured flame.
  \node[inner sep=0pt, outer sep=0pt] at (1.80,4.84)
    {\ethernetcable[width=2.45cm, angle=-41.5, arrow=single,
                    arrow span=0.34]};
  \node[inner sep=0pt, outer sep=0pt] at (2.30,5.56)
    {\recipe[-41.5]{gameorange}};

  % Only after receiving the recipe does B submit the quantum state.
  \node[inner sep=0pt, outer sep=0pt] at (0.25,1.68)
    {\opticfiber[width=5.15cm, image height=0.35cm,
                 angle=-156, arrow=single,
                 arrow span=0.35]};
  \node[inner sep=0pt, outer sep=0pt] at (0.30,2.47)
    {\rotatebox{24}{\scalebox{0.72}{\firestate{gameorange}}}};

  \node[align=center] at (-3.05,-1.28) {%
    $\yoavgameverify\!\left(
      \coloredsquare{gameorange},\;
      \firestate{gameorange}
    \right)=\rejecticon$};

  % Shared convention: time progresses from top to bottom.
  \node[anchor=north, inner sep=0pt, outer sep=0pt] at (5.35,7.50)
    {\timearrow[8.30cm]};
\end{tikzpicture}
\endgroup


==> figs/images/fire-syntax/fire-syntax-figure.tex <==
% Reusable quantum-fire syntax body.
\begingroup
\newcommand{\yoavfirespark}{\mathpzc{Spark}}
\newcommand{\yoavfireclone}{\mathpzc{Clone}}
\newcommand{\yoavfireverify}{\mathpzc{Verify}}
\newcommand{\yoavfireverdict}{\accepticon\;/\;\rejecticon}
\definecolor{fireorange}{RGB}{242,122,24}

% A tabular keeps the small TikZ primitives out of a nested TikZ matrix.
\begin{tabular}{@{}l@{\hspace{1.2em}}c@{\hspace{1.2em}}l@{}}
  $\left(\,\coloredsquare{fireorange}\,,\;\firestate{fireorange}\,\right)$
    & $\longleftarrow$
    & $\yoavfirespark$ \\[4.5ex]
  $\firestate{fireorange}\;\firestate{fireorange}$
    & $\longleftarrow$
    & $\yoavfireclone\!\left(\coloredsquare{fireorange},\;\firestate{fireorange}\right)$ \\[4.5ex]
  \yoavfireverdict
    & $\longleftarrow$
    & $\yoavfireverify\!\left(\coloredsquare{fireorange},\;\firestate{fireorange}\right)$ \\
\end{tabular}
\endgroup


==> figs/images/legend/legend-figure.tex <==
% Reusable legend body, shared by the standalone preview and the main paper.
\begingroup
\definecolor{legendblue}{RGB}{45,55,210}

\newcommand{\yoavlegendanyicon}{\tikz[baseline=-0.5ex]{%
  \draw[black!45, line width=0.4pt, densely dotted, rounded corners=0.03cm]
    (-0.15,-0.15) rectangle (0.15,0.15);}}
\newcommand{\yoavlegendket}[1]{\ensuremath{\left|\,#1\,\right\rangle}}

% A tabular avoids nesting the cable TikZ pictures in a TikZ matrix.
\begin{tabular}{@{}l@{\hspace{1.4em}}l@{}}
  \coloredsquare{legendblue} & a public key or a serial number (a classical string) \\[1.1ex]
  \yoavlegendket{\yoavlegendanyicon} & a quantum state \\[1.1ex]
  \ethernetcable[arrow=double] & a two-way classical channel \\[1.1ex]
  \opticfiber[arrow=single] & a one-way quantum channel \\
\end{tabular}
\endgroup


==> figs/images/oss-security-game/oss-security-game-figure.tex <==
% Reusable one-shot-unforgeability game body.
\begingroup
\newcommand{\yoavgameversign}{\mathsf{VerSign}}
\newcommand{\yoavossgamenote}[1]{\vcenter{\hbox{\signedmessage{ossblue}{#1}}}}
\definecolor{ossblue}{RGB}{45,55,210}

\begin{tikzpicture}
  % Level 1: the adversary.
  \node[draw=black!35, fill=white, rounded corners=1.5pt,
        inner sep=1.5pt, outer sep=0pt] (advA) at (0,6.65)
    {\includegraphics[height=1.50cm]{\yoavdatapath boyPirate}};
  \node[anchor=south, font=\yoavlabeltext] at (advA.north)
    {Adversary $\mathcal A$};

  % Level 2: A's proposed public key and two signed messages.
  \node (proposal) at (0,4.15) {$\left(
    \coloredsquare[0.36cm]{ossblue},\;
    \signedmessage{ossblue}{Hi},\;
    \signedmessage{ossblue}{Bye}
  \right)$};
  \draw[-{Stealth[length=2.8mm,width=2.0mm]}, line width=0.7pt]
    (0,5.78) -- (proposal.north);

  % The crossed arrow marks the computationally hard transition.
  \coordinate (barrier) at (0,2.70);
  \draw[-{Stealth[length=2.8mm,width=2.0mm]}, line width=0.7pt]
    (proposal.south) -- (0,2.15);
  \draw[red!75!black, line width=1.15pt]
    (-0.27,2.52) -- (0.27,2.88);
  \node[anchor=west, align=center, font=\yoavlabeltext, text=red!75!black]
    at (0.42,2.70)
    {computationally\\[-2pt] hard};

  % Level 3: the two formal verification computations.
  \node (checks) at (0,1.10) {$
    \yoavgameversign\!\left(
      \coloredsquare{ossblue},\;\yoavossgamenote{Hi}
    \right)\;\boldsymbol{\wedge}\;
    \yoavgameversign\!\left(
      \coloredsquare{ossblue},\;\yoavossgamenote{Bye}
    \right)$};

  % A successful pair of checks is the hard-to-reach outcome.
  \node (accept) at (-5.55,1.10) {\scalebox{1.25}{\accepticon}};
  \draw[-{Stealth[length=2.8mm,width=2.0mm]}, line width=0.7pt]
    (checks.west) -- (accept.east);

  \node[anchor=north, inner sep=0pt, outer sep=0pt] at (5.65,7.45)
    {\timearrow[6.35cm]};
\end{tikzpicture}
\endgroup


==> figs/images/oss-syntax/oss-syntax-figure.tex <==
% Reusable one-shot-signature syntax body.
\begingroup
\newcommand{\yoavossgen}{\mathpzc{KeyGen}}
\newcommand{\yoavosssign}{\mathpzc{Sign}}
\newcommand{\yoavossversign}{\mathsf{VerSign}}
\newcommand{\yoavossvertoken}{\mathpzc{VerToken}}
\newcommand{\yoavossket}[1]{\left|\,#1\,\right\rangle}
\newcommand{\yoavossverdict}{\accepticon\;/\;\rejecticon}
\definecolor{ossblue}{RGB}{45,55,210}

% A tabular keeps the small TikZ primitives out of a nested TikZ matrix.
\begin{tabular}{@{}l@{\hspace{1.2em}}c@{\hspace{1.2em}}l@{}}
  $\coloredsquare{ossblue}\,,\;\yoavossket{\signingstamp{ossblue}}$
    & $\longleftarrow$
    & $\yoavossgen$ \\[7ex]
  \signedmessage{ossblue}{Hi}
    & $\longleftarrow$
    & $\yoavosssign\!\left(\yoavossket{\signingstamp{ossblue}},\;\mathrm{Hi}\right)$ \\[7ex]
  \yoavossverdict
    & $\longleftarrow$
    & $\yoavossversign\!\left(\coloredsquare{ossblue},\;\signedmessage{ossblue}{Hi}\right)$ \\[7ex]
  \yoavossverdict
    & $\longleftarrow$
    & $\yoavossvertoken\!\left(\coloredsquare{ossblue},\;\yoavossket{\signingstamp{ossblue}}\right)$ \\
\end{tabular}
\endgroup


==> figs/primitives/approved-imprint.tex <==
% =============================================================================
% \approvedimprint — a colourable rendering of data/approved.png.
%
%   \approvedimprint{blue}
%   \approvedimprint[0.8cm]{orange}
%
%   #1 (optional) width of the imprint                         (default 0.7cm)
%   #2            any colour understood by xcolor/TikZ
%
% The source PNG is black with a transparent background.  It is inverted only
% while building a TikZ opacity mask; the command then fills that mask with the
% requested colour.  This keeps the original antialiased edge and supports
% arbitrary colours without needing one recoloured PNG per figure.
%
% Requirements: graphicx, xcolor, and tikz with the fadings library.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}

\ifdefined\approvedimprint\else
  \begin{tikzfadingfrompicture}[name=yoav approved imprint mask]
    \node[inner sep=0pt, outer sep=0pt] {\includegraphics[
      width=1cm,
      decodearray={1 0 1 0 1 0}
    ]{\yoavdatapath approved}};
  \end{tikzfadingfrompicture}

  \NewDocumentCommand{\approvedimprint}{O{0.7cm} m}{%
    \tikz[baseline=-0.5ex]{%
      \pgfmathsetlengthmacro{\yoavimprinthalf}{0.5*(#1)}%
      \path[use as bounding box]
        (-\yoavimprinthalf,-\yoavimprinthalf)
        rectangle
        ( \yoavimprinthalf, \yoavimprinthalf);
      \path[fill=#2, path fading=yoav approved imprint mask]
        (-\yoavimprinthalf,-\yoavimprinthalf)
        rectangle
        ( \yoavimprinthalf, \yoavimprinthalf);
    }%
  }
\fi


==> figs/primitives/ethernet-cable.tex <==
% =============================================================================
% \ethernetcable — an ethernet cable, standing for a classical channel.
%
% The drawing is figs/data/ethernet.png, overlaid with an arrow
% along the middle of its tube saying which way the channel runs.
%
%   \ethernetcable                          % default: 3.2cm wide, two-way
%   \ethernetcable[arrow=double]            % top ->, bottom <-
%   \ethernetcable[angle=30]                % rotated 30 degrees counter-clockwise
%   \ethernetcable[width=5cm, angle=-15, arrow=none]
%
% Options
%   width        the cable's length before rotation         (default 3.2cm)
%   image height fixed artwork height; setting this stretches only length
%                                                            (default auto)
%   angle        rotation, counter-clockwise degrees        (default 0)
%   arrow        none | single | reverse | double           (default single)
%   arrow color                                             (default black)
%   arrow span   fraction of the width the arrow covers     (default 0.44)
%   arrow scale  enlarges or shrinks the whole arrow        (default 1)
%   line width   the arrow's weight                         (default auto)
%   tip length   the arrowhead's length                     (default auto)
%   tip width    the arrowhead's width                      (default auto)
%
% ARROW SIZING. The arrow has to fit inside the tube, so its auto sizes are
% derived from the tube's thickness and not from the cable's width: this
% artwork's tube measures 0.0628 of the image width, whereas the other cable's
% is thicker or thinner, so a shared ratio would overflow one of them. Give
% any of the three keys a length to override, or use arrow scale to keep the
% proportions and just change the size.
%
% The image is turned by graphicx, with origin=c so that it pivots about its
% own centre, and the arrow is turned by the same angle. width must precede
% angle, since graphicx applies its keys in order: angle first would rotate,
% then scale the rotated bounding box to the given width.
%
% CAVEAT. Do not use this command inside a cell of a tikz "matrix of nodes":
% nesting a tikzpicture in a matrix cell displaces the inner picture's nodes
% relative to its paths, so the cable slides off its arrow. This is a TikZ
% limitation, reproducible with any nested picture, not something this command
% can work around. A tabular row holds it correctly, which is what the legend
% uses.
%
% Requirements: graphicx, and tikz with the arrows.meta library. When
% compiling from anywhere but the repository root, point \yoavdatapath at the
% data directory first, e.g. \renewcommand{\yoavdatapath}{../data/}.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}
\def\yoavcableauto{auto}
\def\yoavcablemodenone{none}
\def\yoavcablemodesingle{single}
\def\yoavcablemodereverse{reverse}
\def\yoavcablemodedouble{double}

% The keys below are shared by every cable primitive, so each file sets them
% up; the definitions are identical and simply overwrite one another. Anything
% that differs between cables — the default arrow, the tube thickness — is set
% inside the command body instead, so that two primitives sharing this family
% cannot clobber each other's values.
\pgfkeys{
  /yoav/cable/.is family, /yoav/cable,
  width/.store in=\yoavcablewidth,
  image height/.store in=\yoavcableimageheight,
  angle/.store in=\yoavcableangle,
  arrow color/.store in=\yoavcablearrowcolor,
  arrow span/.store in=\yoavcablearrowspan,
  arrow scale/.store in=\yoavcablearrowscale,
  line width/.store in=\yoavcablelinewidth,
  tip length/.store in=\yoavcabletiplength,
  tip width/.store in=\yoavcabletipwidth,
  arrow/.is choice,
  arrow/none/.code={\def\yoavcablearrowmode{none}\def\yoavcabletips{}\def\yoavcablehasarrow{0}},
  arrow/single/.code={\def\yoavcablearrowmode{single}%
                      \def\yoavcabletips{-{Stealth[length=\yoavcabletl,width=\yoavcabletw]}}%
                      \def\yoavcablehasarrow{1}},
  arrow/reverse/.code={\def\yoavcablearrowmode{reverse}%
                       \def\yoavcabletips{{Stealth[length=\yoavcabletl,width=\yoavcabletw]}-}%
                       \def\yoavcablehasarrow{1}},
  arrow/double/.code={\def\yoavcablearrowmode{double}\def\yoavcabletips{}%
                      \def\yoavcablehasarrow{1}},
  defaults/.style={width=3.2cm, image height=auto, angle=0,
                   arrow color=black, arrow span=0.44,
                   arrow scale=1, line width=auto, tip length=auto,
                   tip width=auto},
}

\ifdefined\ethernetcable\else
\NewDocumentCommand{\ethernetcable}{O{}}{%
  \begin{tikzpicture}[baseline=-0.5ex]
    \pgfkeys{/yoav/cable, defaults, arrow=double, #1}
    % this artwork's tube thickness, as a fraction of the image width
    \def\yoavcabletube{0.0628}
    \pgfmathsetlengthmacro{\yoavarrowhalf}{0.5*\yoavcablearrowspan*\yoavcablewidth}
    \ifx\yoavcableimageheight\yoavcableauto
      \pgfmathsetlengthmacro{\yoavtubethick}{\yoavcabletube*\yoavcablewidth*\yoavcablearrowscale}%
    \else
      % At the source image's aspect ratio, the tube is 0.510 of its height.
      \pgfmathsetlengthmacro{\yoavtubethick}{0.510*\yoavcableimageheight*\yoavcablearrowscale}%
    \fi
    \ifx\yoavcablelinewidth\yoavcableauto
      \pgfmathsetlengthmacro{\yoavcablelw}{0.17*\yoavtubethick}%
    \else\def\yoavcablelw{\yoavcablelinewidth}\fi
    \ifx\yoavcabletipwidth\yoavcableauto
      \ifx\yoavcablearrowmode\yoavcablemodedouble
        \pgfmathsetlengthmacro{\yoavcabletw}{0.44*\yoavtubethick}%
      \else
        \pgfmathsetlengthmacro{\yoavcabletw}{0.68*\yoavtubethick}%
      \fi
    \else\def\yoavcabletw{\yoavcabletipwidth}\fi
    \ifx\yoavcabletiplength\yoavcableauto
      \pgfmathsetlengthmacro{\yoavcabletl}{1.30*\yoavcabletw}%
    \else\def\yoavcabletl{\yoavcabletiplength}\fi
    \pgfmathsetlengthmacro{\yoavcablearrowoffset}{0.19*\yoavtubethick}
    \node[inner sep=0pt, outer sep=0pt] at (0,0) {%
      \ifx\yoavcableimageheight\yoavcableauto
        \includegraphics[width=\yoavcablewidth, angle=\yoavcableangle,
                         origin=c]{\yoavdatapath ethernet}%
      \else
        \rotatebox[origin=c]{\yoavcableangle}{%
          \resizebox{\yoavcablewidth}{\yoavcableimageheight}{%
            \includegraphics{\yoavdatapath ethernet}}}%
      \fi
    };
    \ifnum\yoavcablehasarrow=1
      \ifx\yoavcablearrowmode\yoavcablemodedouble
        \draw[-{Stealth[length=\yoavcabletl,width=\yoavcabletw]},
              draw=\yoavcablearrowcolor, line width=\yoavcablelw,
              rotate=\yoavcableangle]
          (-\yoavarrowhalf,\yoavcablearrowoffset) --
          ( \yoavarrowhalf,\yoavcablearrowoffset);
        \draw[{Stealth[length=\yoavcabletl,width=\yoavcabletw]}-,
              draw=\yoavcablearrowcolor, line width=\yoavcablelw,
              rotate=\yoavcableangle]
          (-\yoavarrowhalf,-\yoavcablearrowoffset) --
          ( \yoavarrowhalf,-\yoavcablearrowoffset);
      \else
        \draw[\yoavcabletips, draw=\yoavcablearrowcolor,
              line width=\yoavcablelw, rotate=\yoavcableangle]
          (-\yoavarrowhalf,0) -- (\yoavarrowhalf,0);
      \fi
    \fi
  \end{tikzpicture}%
}
\fi


==> figs/primitives/fire.tex <==
% =============================================================================
% \firestate — a colourable quantum-fire state, including its ket.
%
%   \firestate{orange}
%   \firestate{red!80!orange}
%
%   #1  any colour understood by xcolor/TikZ
%
% The source PNG is black with a transparent background and is stored tightly
% cropped to its visible alpha bounds.  Its mask is filled with the requested
% colour.  This retains the PNG's antialiased silhouette without storing
% recoloured copies and prevents an invisible border from enlarging ket
% delimiters.  \fireglyph is the internal image-only form used inside the ket.
%
% Requirements: amsmath, graphicx, xcolor, and tikz with the fadings library.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}

\ifdefined\firestate\else
  \begin{tikzfadingfrompicture}[name=yoav fire mask]
    \node[inner sep=0pt, outer sep=0pt] {\includegraphics[
      width=1cm,
      decodearray={1 0 1 0 1 0}
    ]{\yoavdatapath fire}};
  \end{tikzfadingfrompicture}

  \newcommand{\fireglyph}[1]{%
    \ensuremath{\vcenter{\hbox{\tikz[baseline=0pt]{%
      % Tight 798:1101 aspect ratio matching the visible source artwork.
      \path[use as bounding box] (-0.31,-0.428) rectangle (0.31,0.428);
      \path[fill=#1, path fading=yoav fire mask]
        (-0.31,-0.428) rectangle (0.31,0.428);
    }}}}%
  }

  \newcommand{\firestate}[1]{%
    \ensuremath{\left|\,\fireglyph{#1}\,\right\rangle}%
  }
\fi


==> figs/primitives/illustration-style.tex <==
% =============================================================================
% Shared typography for the Yoav illustrations.
%
% No readable prose inside an illustration should be set below \yoavmintext
% (9pt by default).  Ordinary labels use \yoavlabeltext (10pt by default).
% Define either command before loading this file to override it globally.
% =============================================================================
\providecommand{\yoavmintext}{\fontsize{9pt}{10.5pt}\selectfont}
\providecommand{\yoavlabeltext}{\fontsize{10pt}{12pt}\selectfont}


==> figs/primitives/live-signing-token.tex <==
% =============================================================================
% \livesigningtoken — a one-shot signing-token state with a flame above it.
%
%   \livesigningtoken{blue}{red}
%   \livesigningtokenright{blue}{red}  % flame above-right of the state
%   \livesigningtokenindex{blue}{red}  % flame as a lower-right index
%
%   #1  flame colour (the fire's serial-number identity)
%   #2  signing-token/imprint colour
%
% Load fire.tex and signing-stamp.tex before this file.
% Requirements: amsmath and graphicx.
% =============================================================================
\ifdefined\livesigningtoken\else
\NewDocumentCommand{\livesigningtoken}{m m}{%
  \ensuremath{\vcenter{\hbox{$%
    \overset{\scalebox{0.46}{\fireglyph{#1}}}%
      {\left|\,\signingstamp{#2}\,\right\rangle}%
  $}}}%
}
\fi

\ifdefined\livesigningtokenright\else
\NewDocumentCommand{\livesigningtokenright}{m m}{%
  \ensuremath{\vcenter{\hbox{\tikz[baseline=0pt]{%
    \node[inner sep=0pt, outer sep=0pt] (yoav live token)
      {$\left|\,\signingstamp{#2}\,\right\rangle$};
    \node[inner sep=0pt, outer sep=0pt] at (0.29,0.66)
      {\scalebox{0.46}{\fireglyph{#1}}};
  }}}}%
}
\fi

\ifdefined\livesigningtokenindex\else
\NewDocumentCommand{\livesigningtokenindex}{m m}{%
  \ensuremath{%
    \left|\,\signingstamp{#2}\,\right\rangle_{
      \smash{\scalebox{0.31}{\fireglyph{#1}}}%
    }%
  }%
}
\fi


==> figs/primitives/optic-fiber.tex <==
% =============================================================================
% \opticfiber — an optic fibre, standing for a quantum channel.
%
% The drawing is figs/data/optic.png, overlaid with an arrow
% along the middle of its tube saying which way the channel runs.
%
%   \opticfiber                          % default: 3.2cm wide, one-way
%   \opticfiber[arrow=double]            % top ->, bottom <-
%   \opticfiber[angle=30]                % rotated 30 degrees counter-clockwise
%   \opticfiber[width=5cm, angle=-15, arrow=none]
%
% Options
%   width        the cable's length before rotation         (default 3.2cm)
%   image height fixed artwork height; setting this stretches only length
%                                                            (default auto)
%   angle        rotation, counter-clockwise degrees        (default 0)
%   arrow        none | single | reverse | double           (default double)
%   arrow color                                             (default black)
%   arrow span   fraction of the width the arrow covers     (default 0.44)
%   arrow scale  enlarges or shrinks the whole arrow        (default 1)
%   line width   the arrow's weight                         (default auto)
%   tip length   the arrowhead's length                     (default auto)
%   tip width    the arrowhead's width                      (default auto)
%
% ARROW SIZING. The arrow has to fit inside the tube, so its auto sizes are
% derived from the tube's thickness and not from the cable's width: this
% artwork's tube measures 0.0238 of the image width, whereas the other cable's
% is thicker or thinner, so a shared ratio would overflow one of them. Give
% any of the three keys a length to override, or use arrow scale to keep the
% proportions and just change the size.
%
% The image is turned by graphicx, with origin=c so that it pivots about its
% own centre, and the arrow is turned by the same angle. width must precede
% angle, since graphicx applies its keys in order: angle first would rotate,
% then scale the rotated bounding box to the given width.
%
% CAVEAT. Do not use this command inside a cell of a tikz "matrix of nodes":
% nesting a tikzpicture in a matrix cell displaces the inner picture's nodes
% relative to its paths, so the cable slides off its arrow. This is a TikZ
% limitation, reproducible with any nested picture, not something this command
% can work around. A tabular row holds it correctly, which is what the legend
% uses.
%
% Requirements: graphicx, and tikz with the arrows.meta library. When
% compiling from anywhere but the repository root, point \yoavdatapath at the
% data directory first, e.g. \renewcommand{\yoavdatapath}{../data/}.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}
\def\yoavcableauto{auto}
\def\yoavcablemodenone{none}
\def\yoavcablemodesingle{single}
\def\yoavcablemodereverse{reverse}
\def\yoavcablemodedouble{double}

% The keys below are shared by every cable primitive, so each file sets them
% up; the definitions are identical and simply overwrite one another. Anything
% that differs between cables — the default arrow, the tube thickness — is set
% inside the command body instead, so that two primitives sharing this family
% cannot clobber each other's values.
\pgfkeys{
  /yoav/cable/.is family, /yoav/cable,
  width/.store in=\yoavcablewidth,
  image height/.store in=\yoavcableimageheight,
  angle/.store in=\yoavcableangle,
  arrow color/.store in=\yoavcablearrowcolor,
  arrow span/.store in=\yoavcablearrowspan,
  arrow scale/.store in=\yoavcablearrowscale,
  line width/.store in=\yoavcablelinewidth,
  tip length/.store in=\yoavcabletiplength,
  tip width/.store in=\yoavcabletipwidth,
  arrow/.is choice,
  arrow/none/.code={\def\yoavcablearrowmode{none}\def\yoavcabletips{}\def\yoavcablehasarrow{0}},
  arrow/single/.code={\def\yoavcablearrowmode{single}%
                      \def\yoavcabletips{-{Stealth[length=\yoavcabletl,width=\yoavcabletw]}}%
                      \def\yoavcablehasarrow{1}},
  arrow/reverse/.code={\def\yoavcablearrowmode{reverse}%
                       \def\yoavcabletips{{Stealth[length=\yoavcabletl,width=\yoavcabletw]}-}%
                       \def\yoavcablehasarrow{1}},
  arrow/double/.code={\def\yoavcablearrowmode{double}\def\yoavcabletips{}%
                      \def\yoavcablehasarrow{1}},
  defaults/.style={width=3.2cm, image height=auto, angle=0,
                   arrow color=black, arrow span=0.44,
                   arrow scale=1, line width=auto, tip length=auto,
                   tip width=auto},
}

\ifdefined\opticfiber\else
\NewDocumentCommand{\opticfiber}{O{}}{%
  \begin{tikzpicture}[baseline=-0.5ex]
    \pgfkeys{/yoav/cable, defaults, arrow=single, #1}
    % this artwork's tube thickness, as a fraction of the image width
    \def\yoavcabletube{0.0238}
    \pgfmathsetlengthmacro{\yoavarrowhalf}{0.5*\yoavcablearrowspan*\yoavcablewidth}
    \ifx\yoavcableimageheight\yoavcableauto
      \pgfmathsetlengthmacro{\yoavtubethick}{\yoavcabletube*\yoavcablewidth*\yoavcablearrowscale}%
    \else
      % At the source image's aspect ratio, the tube is 0.295 of its height.
      \pgfmathsetlengthmacro{\yoavtubethick}{0.295*\yoavcableimageheight*\yoavcablearrowscale}%
    \fi
    \ifx\yoavcablelinewidth\yoavcableauto
      \pgfmathsetlengthmacro{\yoavcablelw}{0.17*\yoavtubethick}%
    \else\def\yoavcablelw{\yoavcablelinewidth}\fi
    \ifx\yoavcabletipwidth\yoavcableauto
      \ifx\yoavcablearrowmode\yoavcablemodedouble
        \pgfmathsetlengthmacro{\yoavcabletw}{0.24*\yoavtubethick}%
      \else
        % Keep the arrowhead inside the white bore, rather than merely inside
        % the tube's outer black contour.
        \pgfmathsetlengthmacro{\yoavcabletw}{0.50*\yoavtubethick}%
      \fi
    \else\def\yoavcabletw{\yoavcabletipwidth}\fi
    \ifx\yoavcabletiplength\yoavcableauto
      \pgfmathsetlengthmacro{\yoavcabletl}{1.30*\yoavcabletw}%
    \else\def\yoavcabletl{\yoavcabletiplength}\fi
    \pgfmathsetlengthmacro{\yoavcablearrowoffset}{0.13*\yoavtubethick}
    \node[inner sep=0pt, outer sep=0pt] at (0,0) {%
      \ifx\yoavcableimageheight\yoavcableauto
        \includegraphics[width=\yoavcablewidth, angle=\yoavcableangle,
                         origin=c]{\yoavdatapath optic}%
      \else
        \rotatebox[origin=c]{\yoavcableangle}{%
          \resizebox{\yoavcablewidth}{\yoavcableimageheight}{%
            \includegraphics{\yoavdatapath optic}}}%
      \fi
    };
    \ifnum\yoavcablehasarrow=1
      \ifx\yoavcablearrowmode\yoavcablemodedouble
        \draw[-{Stealth[length=\yoavcabletl,width=\yoavcabletw]},
              draw=\yoavcablearrowcolor, line width=\yoavcablelw,
              rotate=\yoavcableangle]
          (-\yoavarrowhalf,\yoavcablearrowoffset) --
          ( \yoavarrowhalf,\yoavcablearrowoffset);
        \draw[{Stealth[length=\yoavcabletl,width=\yoavcabletw]}-,
              draw=\yoavcablearrowcolor, line width=\yoavcablelw,
              rotate=\yoavcableangle]
          (-\yoavarrowhalf,-\yoavcablearrowoffset) --
          ( \yoavarrowhalf,-\yoavcablearrowoffset);
      \else
        \draw[\yoavcabletips, draw=\yoavcablearrowcolor,
              line width=\yoavcablelw, rotate=\yoavcableangle]
          (-\yoavarrowhalf,0) -- (\yoavarrowhalf,0);
      \fi
    \fi
  \end{tikzpicture}%
}
\fi


==> figs/primitives/recipe.tex <==
% =============================================================================
% \recipe — a paper carrying a coloured flame recipe.
%
%   \recipe{orange}
%   \recipe[-45]{blue!70!black}
%
%   #1 (optional) rotation in degrees                          (default 0)
%   #2            colour of the flame printed on the paper
%
% Requirements: graphicx, xcolor, tikz, and fire.tex loaded first.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}
\providecommand{\yoavmintext}{\fontsize{9pt}{10.5pt}\selectfont}

\ifdefined\recipe\else
\NewDocumentCommand{\recipe}{O{0} m}{%
  \tikz[baseline=-0.5ex, rotate=#1, transform shape]{%
    \path[use as bounding box] (-0.49,-0.60) rectangle (0.49,0.60);
    \node[inner sep=0pt, outer sep=0pt] at (0,0) {\includegraphics[
      width=0.96cm,
      trim=289bp 20bp 292bp 29bp,
      clip
    ]{\yoavdatapath paper}};
    % Fit the complete title inside the usable width below the folded corner.
    \node[anchor=north, inner sep=0pt, outer sep=0pt, text=black]
      at (0,0.43) {\resizebox{0.78cm}{!}{\textbf{Recipe for}}};
    % The recipe shows the bare flame glyph: unlike \firestate, there is no ket.
    \node[inner sep=0pt, outer sep=0pt] at (0,-0.18)
      {\scalebox{0.68}{\fireglyph{#2}}};
  }%
}
\fi


==> figs/primitives/signed-key-pair.tex <==
% =============================================================================
% \signedkeypair — a paper containing two public keys and a coloured seal.
%
%   \signedkeypair{blue}{red}{yellow}
%   \signedkeypair[0.56]{blue}{red}{yellow}  % uniformly scaled
%
%   #1 (optional) uniform scale                              (default 1)
%   #2            colour of the signing/approval seal
%   #3            colour of the left signed key
%   #4            colour of the right signed key
%
% Load approved-imprint.tex before this file.
% Requirements: graphicx, xcolor, and tikz with the fadings library.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}

\ifdefined\signedkeypair\else
\NewDocumentCommand{\signedkeypair}{O{1} m m m}{%
  % Scale the complete TikZ picture here rather than wrapping the command in
  % \scalebox.  Nested raster nodes and vector overlays can otherwise acquire
  % different transforms, visibly pulling the key squares off the paper.
  \tikz[baseline=-0.5ex, scale=#1, transform shape]{%
    \path[use as bounding box] (-0.83,-1.29) rectangle (0.83,0.79);
    % Draw the sheet as part of this picture.  The former cropped PNG could
    % shift relative to the TikZ paths when the certificate was reduced for
    % inline formulas, leaving the left key visibly outside the paper.
    \path[draw=black!32, fill=yellow!5, line width=0.3pt,
          line join=round]
      (-0.82,-1.28) -- (-0.82,0.78) -- (0.58,0.78) --
      (0.82,0.54) -- (0.82,-1.28) -- cycle;
    \path[draw=black!32, fill=yellow!10, line width=0.3pt,
          line join=round]
      (0.58,0.78) -- (0.58,0.54) -- (0.82,0.54) -- cycle;
    \path[draw=#3!60!black, fill=#3, line width=0.3pt]
      (-0.48,0.35) rectangle (-0.18,0.65);
    \path[draw=#4!60!black, fill=#4, line width=0.3pt]
      (0.05,0.35) rectangle (0.35,0.65);
    % Keep the approval seal in this same coordinate system as the sheet.
    % Its centre is fixed on the paper's horizontal axis and its lower edge
    % leaves a small, even margin above the bottom of the page.  Its 1.44 cm
    % square is exactly twice the former 0.72 cm seal and fills nearly all of
    % the lower certificate without touching the key row.
    \path[fill=#2, path fading=yoav approved imprint mask]
  (-1.26,-1.76) rectangle (1.26,0.76);
  }%
}
\fi


==> figs/primitives/signed-message.tex <==
% =============================================================================
% \signedmessage — a paper carrying a message and a coloured approval imprint.
%
%   \signedmessage{blue}{Hi}
%   \signedmessage{orange}{m}
%
%   #1  colour of the APPROVED imprint
%   #2  message printed at the paper's upper left
%
% Load approved-imprint.tex before this file.
% Requirements: graphicx, xcolor, and tikz with the fadings library.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}
\providecommand{\yoavmintext}{\fontsize{9pt}{10.5pt}\selectfont}

\ifdefined\signedmessage\else
\NewDocumentCommand{\signedmessage}{m m}{%
  \tikz[baseline=-0.5ex]{%
    \path[use as bounding box] (-0.79,-0.94) rectangle (0.79,0.94);
    % Remove the source PNG's white staging area while retaining the paper,
    % its folded corner, and the faint shadow around it.
    \node[inner sep=0pt, outer sep=0pt] at (0,0) {\includegraphics[
      width=1.58cm,
      trim=289bp 20bp 292bp 29bp,
      clip
    ]{\yoavdatapath paper}};
    % The message occupies the top quarter of the sheet and never crosses its
    % side borders.  9pt is the global minimum readable illustration size.
    \node[anchor=north, inner sep=0pt, outer sep=0pt,
          text=black, font=\yoavmintext, text width=1.20cm, align=center]
      at (0,0.71) {#2};
    % Exactly twice the former 0.69cm imprint, still inside the paper border.
    \node[inner sep=0pt, outer sep=0pt] at (0,-0.22)
      {\approvedimprint[2.1cm]{#1}};
  }%
}
\fi


==> figs/primitives/signing-stamp.tex <==
% =============================================================================
% \signingstamp — the one-shot signing token: a colourable physical stamp.
%
%   \signingstamp{blue}
%   \signingstamp{orange}
%
%   #1  colour of the stamp
%
% The source PNG is a tightly cropped black alpha mask.  The requested colour
% is painted through that mask, so the token is the coloured stamp itself;
% there is deliberately no APPROVED imprint below it.
%
% Requirements: graphicx, xcolor, and tikz with the fadings library.
% =============================================================================
\providecommand{\yoavdatapath}{figs/data/}

\ifdefined\signingstamp\else
\begin{tikzfadingfrompicture}[name=yoav signing stamp mask]
  \node[inner sep=0pt, outer sep=0pt] {\includegraphics[
    width=1cm,
    decodearray={1 0}
  ]{\yoavdatapath stamp}};
\end{tikzfadingfrompicture}

\NewDocumentCommand{\signingstamp}{m}{%
  \ensuremath{\vcenter{\hbox{\tikz[baseline=0pt]{%
    % Match the cropped artwork's 679:904 aspect ratio and expose no padding
    % to surrounding ket delimiters.
    \path[use as bounding box] (-0.28,-0.373) rectangle (0.28,0.373);
    \path[fill=#1, path fading=yoav signing stamp mask]
      (-0.28,-0.373) rectangle (0.28,0.373);
  }}}}%
}
\fi


==> figs/primitives/square.tex <==
% =============================================================================
% \coloredsquare — the legend's square: a classical string, such as a public
% key or a serial number. The colour is the argument, so that a drawing can
% use colour to tell one string from another.
%
%   \coloredsquare{gray}            % the legend's own use
%   \coloredsquare{blue}
%   \coloredsquare[0.4cm]{orange}   % a larger one
%   \coloredsquare[0.4cm][-45]{orange} % larger and rotated
%
%   #1 (optional) the side length                            (default 0.28cm)
%   #2 (optional) rotation in degrees                        (default 0)
%   #3            the fill colour; the border is drawn in a
%                 darker shade of it
%
% NOTE ON THE NAME. This wants to be called \square, but amssymb defines that
% already and macros.tex uses it as the paper's QED symbol, so taking the name
% would replace the end-of-proof box in every proof. Hence \coloredsquare.
%
% Requirements: tikz. The optional-argument-then-colour shape follows
% \figpk in Claude/figure-C.tex, which draws the same object.
% =============================================================================
\ifdefined\coloredsquare\else
\NewDocumentCommand{\coloredsquare}{O{0.28cm} O{0} m}{%
  \ensuremath{\vcenter{\hbox{\tikz[baseline=0pt, rotate=#2]{%
    \pgfmathsetlengthmacro{\yoavsquarehalf}{0.5*(#1)}%
    \path[fill=#3, draw=#3!60!black, line width=0.3pt]
      (-\yoavsquarehalf,-\yoavsquarehalf)
      rectangle
      ( \yoavsquarehalf, \yoavsquarehalf);}%
  }}}%
}
\fi


==> figs/primitives/time-arrow.tex <==
% =============================================================================
% \timearrow — a reusable top-to-bottom time-direction indicator.
%
%   \timearrow          % 5 cm tall
%   \timearrow[6.5cm]   % custom height
%
% Requirements: tikz with the arrows.meta library.
% =============================================================================
\providecommand{\yoavlabeltext}{\fontsize{10pt}{12pt}\selectfont}

\ifdefined\timearrow\else
\NewDocumentCommand{\timearrow}{O{5cm}}{%
  \tikz[baseline=(current bounding box.center)]{%
    \draw[-{Stealth[length=2.8mm,width=2.0mm]}, line width=0.7pt]
      (0,0) -- node[midway, right=11pt, rotate=-90, font=\yoavlabeltext] {time}
      (0,-#1);
  }%
}
\fi


==> figs/primitives/verdict-icons.tex <==
% =============================================================================
% Parameterless verification verdicts used by the OSS syntax illustration.
%
%   \accepticon   % green circled check
%   \rejecticon   % red circled cross
%
% Requirements: xcolor and tikz.
% =============================================================================
\definecolor{yoavacceptgreen}{RGB}{48,165,55}
\definecolor{yoavrejectred}{RGB}{203,48,43}

\ifdefined\accepticon\else
\newcommand{\accepticon}{%
  \tikz[baseline=-0.5ex]{%
    \fill[yoavacceptgreen!55!black] (0,0) circle (0.22);
    \fill[white] (0,0) circle (0.188);
    \fill[yoavacceptgreen] (0,0) circle (0.158);
    \draw[white, line width=1.0pt, line cap=round, line join=round]
      (-0.070,0.005) -- (-0.022,-0.060) -- (0.082,0.070);
  }%
}
\fi

\ifdefined\rejecticon\else
\newcommand{\rejecticon}{%
  \tikz[baseline=-0.5ex]{%
    \fill[yoavrejectred!55!black] (0,0) circle (0.22);
    \fill[white] (0,0) circle (0.188);
    \fill[yoavrejectred] (0,0) circle (0.158);
    \draw[white, line width=1.0pt, line cap=round]
      (-0.065,-0.065) -- (0.065,0.065)
      (-0.065,0.065) -- (0.065,-0.065);
  }%
}
\fi

